Fair Coexistence of Scheduled and Random Access Wireless Networks: Unlicensed LTE/WiFi

We study the fair coexistence of scheduled and random access transmitters sharing the same frequency channel. Interest in coexistence is topical due to the need for emerging unlicensed LTE technologies to coexist fairly with WiFi. However, this interest is not confined to LTE/WiFi as coexistence is likely to become increasingly commonplace in IoT networks and beyond 5G. In this article we show that mixing scheduled and random access incurs and inherent throughput/delay cost, the cost of heterogeneity. We derive the joint proportional fair rate allocation, which casts useful light on current LTE/WiFi discussions. We present experimental results on inter-technology detection and consider the impact of imperfect carrier sensing.

==> Figures/carriersense.tex <==
\section{Addressing Imperfect Inter-Tech Detection}\label{sec:carrier_sense}

One of the main assumptions in our analysis is that random access nodes are able to detect ongoing transmissions from scheduled nodes, so they defer their channel attempts during $T_{\rm on}$. However, when different technologies coexist, they may use different PHY layers, which questions the validity of this assumption. In this section, we consider the case of real hardware implementing an WiFi/LTE coexistence scenario and evaluate this detection ability. 

%, . We evaluate in this section to what extent this assumption holds for the case where the PHY of  coexisting networks  differ, as it occurs in an unlicensed LTE/WiFi coexisting scenario. \textbf{*CC - to decide - In other scenarios, such as in coexisting TSCH and random access 802.15.4e networks where they both follow the specifications of the 802.15.4e physical layer, we expect this assumption to be accurate.}

%\textbf{*CC Here the flow might be: motivation detection might be erroneous, show in LTE/WiFi case, modify general model accordingly, suggest use of explicit communication, then revisit example with CTS-to-self. Is that too back-and-forth between the general and the technology-specific? If so, can do we do better?}

%\textbf{*CC For the opportunistic approach we need that txA detects random access but we are not saying anything of when that is not the case. Should we at least say that if that is the case, then the preemptive approach is preferred? Or that we should ensure this by other means? Maybe in Scope?}

%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Transmission detection with 802.11}

%\textbf{*CC: TODO: this section needs change according to changes before/after}

%\textbf{**add intro explaining how carrier sense works: in wifi there are three types (i) virtual carrier sense via NAV, (ii) weak carrier sense by correlating with preamble, (iii) energy based carrier sensing with -50dBm threshold (or whatever).  The point being that (iii) is much less sensitive that the other two, and we'll then bring that out in our experimental measurements.}.  


In 802.11 interfaces, the ability to detect ongoing transmissions, namely, ``carrier sensing'', is carried out by two functions: Clear Channel Assessment (CCA) and Virtual Carrier Sensing. \textbf{CCA} is typically built-in in hardware and evaluates if the channel is busy at a particular point in time through two schemes, Preamble Correlation (PC) and Energy Detection (ED). The PC function attempts to decode the preamble of WiFi frames and, when successful, the channel is marked as \empty{busy} for the duration of the transmission as indicated in the preamble. The ED function simply measures the energy in the current frequency range, and triggers a positive detection if the measurement overpasses a threshold. 


%In reality, manufacturers implement different detection techniques to implement a more robust PC function. 
%See, as an example, the signal detection logic of an off-the-shelf Atheros WiFi card in Fig.~\ref{fig:atheros_cca} (\textbf{*AGS: TBD do we want this figure? If so, I will re-do properly}). This radio chipset implements PC running two detection algorithms concurrently \cite{atheros_cca}: a strong signal detector triggers a positive detection upon sudden changes in the received signal power and a more classic approach based on preamble correlation, and an ED based on a -62dBm-threshold. 
%\begin{figure}[hht!] 
%\centering
%\includegraphics[width=\columnwidth]{./Figures/atheros.eps}
%\caption{xxx.\textbf{**Atheros signal detection logic. To re-do if we want it}. More details in \cite{atheros_cca}. }
%\label{fig:atheros_cca}
%\end{figure}


In contrast to CCA, \textbf{Virtual Carrier Sensing} operates at the MAC layer and attempts to reserve the medium for a certain amount of time;  information which is provided in a \emph{duration} field in the MAC header of a transmitted frame. Upon proper decoding of this header, receivers set a Network Allocation Vector (NAV) timer accordingly to mark the channel as busy for the duration requested in the transmitted frame. This is typically used to ``reserve'' the medium for transmissions that might not be properly detected by all stations in the WLAN due to radio conditions, i.e., in scenarios with ``hidden nodes'' when using the RTS/CTS (Ready-to-send/Clear-to-send) message exchange \cite{rtscts}.


In general, ED is less sensitive than PC and virtual carrier sensing, as it builds on energy measurements instead of decoded information, and therefore prone to false negatives. This is of particular interest for our case, as LTE-U and WiFi have different PHY layers and therefore the later might not be able to properly detect the former but via ED e.g. in scenarios where the interfering LTE-U  signal power is not too high. 




% - TX counts the number of cycles the transmission unit is active.
% - RX  is incremented only if any of the two signal detection block outputs is positive. (see fig. attached -- got it from [1] which is a nice reference if you wanna understand how atheros does carrier sensing, e.g. there are 4 blocks to detect the presence of signals each with its own parameter)
% - BUSY counter is the sum of the TX register value, the RX register value *and* the sampled output of the energy detection block (not recognizable packets).


% To assess the effectiveness of carrier sensing using real equipment, we deploy a small test-bed composed of commercial, off-the-shelf devices to set up two links, one WiFi and one LTE, operating in the same 5~GHz channel and using the same bandwidth, namely, 20~MHz. The LTE link consists of two USRP~B210 boards from Ettus connected via an USB~3.0 interface to a standard PCs (Intel Core i7) running Linux Ubuntu Trusty, with the \texttt{uhd\_driver} and version 1.0.0 of \texttt{srsLTE},\footnote{\url{https://github.com/srsLTE/srsLTE}} which is a free and open-source LTE library for SDR UE and eNodeB. The WiFi nodes are Soekris net6501-70 devices running Linux Ubuntu (kernel 3.13), equipped with an Atheros~AR9390-based 802.11a card that is controlled with the \texttt{ath9k} driver. 
% 
% %All devices are placed in a X $\times$ X table.
% 
% We next describe the operation of the wireless links. For the case of LTE,  one device acts as eNodeB, configured to use 100~physical resource blocks and implementing a periodic duty-cycle channel access scheme, similar to the proposed CSAT coexistence mechanism \cite{sadek2015extending}. More specifically, we modify the \texttt{srsLTE} example program \texttt{src/examples/pdsch\_enodeb.c} to fix an active interval during which data is transmitted to the other device, which acts as UE, followed by a silence period of random duration.
% %\footnote{Randomising the LTE silent period alleviates potential quantisation effects~\cite{cano2015unlicensed}.} <- this is explained in this paper.
% The average total duration of the active plus silent periods is equal to 150~ms, and by varying the mean duration of the silent period we can vary the ``duty cycle''  of the LTE link. Throughout our experiments we will also vary the LTE transmission power.
% 
% For the case of WiFi, one of the stations is configured as an Access Point, and the other is associated with it. The former is constantly backlogged with 1500~Bytes UDP frames addressed to the latter, and both use a 17~dBm transmit power. Throughout the experiments we vary the modulation and coding scheme (MCS) used to analyse its impact. Furthermore, we take advantage of \texttt{ath9k} driver's monitoring capabilities to obtain the status of the medium as detected by the wireless card. 
% This is done by leveraging \texttt{ath9k}'s 32-bit register counters \texttt{AR\_CCCNT},  \texttt{AR\_RCCNT}, \texttt{AR\_RFCNT}, and \texttt{AR\_TFCNT}, which counts time at 44~MHz resolution (cycles), number of cycles the card's CCA scheme detects channel as busy state, card is receiving, and card is transmitting, respectively. 
% With this data, we are able to measure what we denote as the ``CCA state'' of the wireless medium. Similar approach is done by \texttt{RegMon}\cite{regmon}.
% 
% We analyse the ability of WiFi's carrier sensing to detect ongoing LTE transmissions by performing a sweep on LTE's duty cycle and transmission power, and measuring WiFi's throughput for each considered configuration during 10~s. More specifically, we compute the relative throughput, this being defined as the ratio between the obtained throughput over the one obtained with no LTE activity, to support comparison across different MCS. We note that, in case carrier sensing is effective to detect ongoing transmissions, this relative throughput should correspond to approximately one minus LTE's duty cycle. 
% 
% The obtained results are depicted in Fig.~\ref{fig:cca_exp}, were we use points to represent the relative throughput, and coloured bars for the CCA state (although we depict results corresponding to a single measurement, we repeated the experiments a number of times and results where very similar in all cases). TO BE CONTINUED. 


%\begin{figure}[hht!] 
%\centering
%\includegraphics[width=0.70\columnwidth]{./Figures/cca_experiment.eps}
%\caption{xxx.}
%\label{fig:cca_exp}
%\end{figure}


\subsection{Testbed and Results}


We deploy a small test-bed to assess the ability of WiFi devices to detect LTE-U activity, by generating different patterns of LTE-U traffic, and gathering the statistics from the clear channel assessment (CCA) module of the WiFi card. 

The LTE-U traffic is generated with an USRP~B210 board from Ettus, connected via an USB~3.0 interface to a standard PCs (Intel Core i7) running Linux Ubuntu Trusty, with the \texttt{uhd\_driver} and version 1.0.0 of \texttt{srsLTE},\footnote{\url{https://github.com/srsLTE/srsLTE}} which is a free and open-source LTE library for SDR UE and eNodeB. The node acts as eNodeB, configured to use 100~physical resource blocks (i.e., 20~MHz bandwidth) in the 5~GHz band and implementing a periodic duty-cycle channel access scheme, similar to the proposed CSAT coexistence mechanism \cite{sadek2015extending}. To this aim, we modify the \texttt{srsLTE} example program \texttt{src/examples/pdsch\_enodeb.c} to fix an active interval during which data is transmitted, followed by a silence period of random duration. The average total duration of the active plus silent periods is equal to 100~ms, and by varying the mean duration of the silent period we can vary the ``duty cycle''  of the LTE link. Throughout our experiments we will also vary the LTE transmission power.

The WiFi channel sensing is performed by a Soekris net6501-70 device equipped with an Atheros~AR9390-based 802.11a card, running Linux Ubuntu (kernel 3.13) and the \texttt{ath9k} wireless driver. We take advantage of this driver's monitoring capabilities to obtain the status of the medium as detected by the wireless card. This is done by leveraging \texttt{ath9k}'s 32-bit register counters \texttt{AR\_CCCNT}, \texttt{AR\_RCCNT}, and \texttt{AR\_RFCNT}, which count, respectively, the total number of cycles elapsed (with a 44~MHz resolution), the ones the medium is marked as busy and the ones there is an ongoing frame. With this data, we are able to measure what we denote as the ``CCA state'' of the wireless medium (a similar approach is done by \texttt{RegMon}\cite{regmon}). 

We plot in Fig.~\ref{fig:cca_exp} (top) the resulting ``CCA state'' for different configurations of the LTE-U duty cycle, MCS index 0, and two values of the transmission power. We start by analysing the -16~dBm case. We note that, given the small size of the testbed, for this configuration the signal quality in close proximity was very good (we confirmed this with another Ettus board, configured as LTE-U UE). However, according to the results obtained, the WiFi card fails to mark the medium as busy for all duty cycles: even for the case of 80\% of activity, the card marks the medium as idle for (approx.) 95\% of the time. On the other hand, when the transmission power is high (the 4~dBm case), the amount of time the card marks the medium as busy follows the duty cycle values. 

To check if the above was caused by hardware issues from the Ettus card, we repeat the experiment but running an IEEE 802.11a transceiver\footnote{\url{https://github.com/bastibl/gr-ieee802-11}} over the USRP~B210 board, generating a similar transmission pattern in the same frequency and using the 6~Mbps MCS (which is the closest 802.11-compliant modulation to that of the LTE-U experiment). In order to generate similar patterns as our SDR LTE experiment we transmit WiFi packets in bursts during the ``on'' periods (without idle time between two packets, i.e. no DIFS and no random backoff), and remain silent during a random ``off'' periods. The ``CCA state'' for this set of experiments is depicted in Fig.~\ref{fig:cca_exp} (bottom), where we confirm that the WiFi card correctly detects that the medium is occupied by 802.11 transmissions for both values of the transmission power, closely following the duty cycle. Based on these results, we conclude that the channel assessment scheme of existing WiFi devices is not well suited for the coexistence of LTE-U and WiFi. 

\begin{figure}[hht!] 
\centering
\includegraphics[width=\columnwidth]{./Figures/wifi_lte_comparison.eps}
\caption{WiFi Atheros CCA states with  an SDR LTE-U implementation (top), and  an SDR 802.11a implementation (bottom). }
\label{fig:cca_exp}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Enabling Explicit Communication}

As we have seen above, correct detection via carrier sensing of a scheduled transmission by the random access network cannot be assumed perfect when the PHY differ. One solution to overcome this is to enable explicit communication. That is, enabling the scheduled network to transmit a signal decodable by the random access network at the start of a $T_{\rm on}$ period, announcing the duration of the transmission. By successfully receiving this signal, a CSMA/CA transmitter will be able to defer its transmissions until the start of the next $T_{\rm off}$ interval. Thus, relying in virtual detection instead of in indirect detection by carrier sensing.

A drawback of explicit communication is the fact that the explicit signaling is prone to loss. A clear example of this is when a collision occurs between transmitters $A$ and $B$ at the start of a $T_{\rm on}$ period, where this signal should be transmitted. In this case, transmitters $B$ may be incapable of correctly decoding this signal and thus, enable to defer transmission accordingly. We evaluate here how the performance of the network varies for both of the approaches presented before (\emph{Preemptive} and \emph{Opportunistic}) when explicit communication is enabled and is prone to be lost due to collisions between transmitters $A$ and $B$ at the start of the $T_{\rm on}$.  

%in a heterogeneous scenario is for the LTE network to transmit a WiFi-like signal at the start of the transmission to allow WiFi devices to deem the medium busy and to determine the LTE transmission duration. A practical way to implement this is the use of 802.11 CTS-to-self frames as proposed in \cite{sadek2015extending}. However, a drawback of this approach is the impossibility to decode this frame when when facing a WiFi/LTE collision. Thus, when a WiFi/LTE collision occurs, there is the potential for WiFi to transmit multiple packets during the LTE $T_{\rm on}$ time, considerably degrading LTE throughput. We evaluate here how the performance of the network varies for both CSAT and LBE in this case. 

\subsection{Throughput Model with Explicit Communication}\label{sec:appendix_model_imperfectcs}

We can easily extend the throughput analysis in Section \ref{sec:appendix_model} to the case in which CSMA/CA transmitters can only detect transmissions from transmitter $A$ when there is not a collision at the start of the $T_{\rm on}$ period.  

\subsubsection{\textbf{CSMA/CA Throughput}}

Note that it does not affect CSMA/CA throughput whether transmitters $B$ \emph{(i)} continue to transmit during $T_{\rm on}$ due to the impossibility of receiving the explicit signaling or \emph{(ii)} defer to transmitter $A$. In \emph{(i)} CSMA/CA stations will suffer from collisions with the scheduled transmitter and in \emph{(ii)} CSMA/CA transmitters are not allowed to transmit due to detection and deferral. Thus, there is no contribution to throughput in either case. However, using both the \emph{Preemptive} and the \emph{Opportunistic} approaches, there can now be a partial collision at the end of the $T_{\rm on}$ period that extends beyond the scheduled transmission duration. Thus, affecting the value of $\E[\hat{T}_{{\rm off}}]$.

\paragraph{\textbf{Preemptive Approach}}

Assuming, similarly as for the collisions at the start of the scheduled transmission, that on average the collisions at the end of the $T_{\rm on}$ period occur half-way through the CSMA/CA transmissions and that these collisions occur also with probability $p_{{\rm txA}} = \frac{(1-p_{\rm e})\Delta }{\E[M]}$, then:

\small
\begin{align}
\E[\hat{T}_{{\rm off}}]=\bar{T}_{{\rm off}} - \frac{\Delta}{2}p_{{\rm txA}}(1-p_{{\rm txA}}) - \Delta p_{{\rm txA}}^2.\label{eq:newToff}
\end{align}
\normalsize

Where we also assume that the collision probability at the start of the $T_{\rm on}$ is independent of the probability at the end of $T_{\rm on}$, which should hold when $T_{\rm on} >> \Delta$.

\paragraph{\textbf{Opportunistic Approach}} 

In the \emph{Opportunistic} approach there will still not be partial collisions at the start of the $T_{\rm on}$ period but there is potential for these to occur at the end of the $T_{\rm on}$ if CSMA/CA stations continue to transmit due to the impossibility to receive the explicit signaling. Thus, $\E[\hat{T}_{{\rm off}}]$ is no longer equal to $\E[T_{{\rm off}}]$, instead we have:

\small
\begin{align}
\E[\hat{T}_{{\rm off}}]=\bar{T}_{{\rm off}} - \frac{\Delta}{2}(1-p_{\rm e})p_{{\rm txA}},
\end{align}
\normalsize

with $p_{{\rm txA}} = \frac{(1-p_{\rm e})\Delta }{\E[M]}$ as in the \emph{Preemptive} approach.

\subsubsection{\textbf{Resulting Throughput for the Scheduled Network}}

We assume in the following that the maximum idle space left between random access transmissions is smaller than a full slot ($\delta$). Thus, when a collision occurs at the beginning of the $T_{\rm on}$, the multiple transmissions of CSMA/CA stations will corrupt all frames sent by transmitter $A$.

\paragraph{\textbf{Preemptive Approach}}

In this case, the resulting throughput for the scheduled network can be rewritten simply as:

\begin{align}
s_{{\rm txA}} =r\frac{T_{\rm on}(1-p_{{\rm txA}})} {T_{\rm on}+\bar{T}_{{\rm off}}}.
\end{align}

\paragraph{\textbf{Opportunistic Approach}} 

Similarly, for the \emph{Opportunistic} approach we can compute the resulting scheduled throughput as:

\small
\begin{align}
s_{{\rm txA}} &=r\frac{(T_{\rm on} - T_{\rm res})(1-p_{{\rm txA}})}{T_{\rm on}+\bar{T}_{{\rm off}}}.
\end{align}
\normalsize

%\subsection{Example: Unlicensed LTE and WiFi with CTS-to-self}
\subsection{Example: LTE-U and WiFi with Virtual Carrier Sensing}

The use of explicit communication in the context of unlicensed LTE and WiFi has been proposed in \cite{sadek2015extending}. In that work, the CTS-to-self (a 802.11 frame) is used by LTE as a practical way to ensure correct detection of LTE transmissions by WiFi. 

% As discussed before, if LTE uses explicit communication such as the CTS-to-self before transmission, we assume WiFi will correctly detect LTE transmissions and so defer its channel attempts during the $T_{\rm on}$. However, that only occurs when LTE and WiFi do not collide at the start of the $T_{\rm on}$ period. 

 
We show in Figure \ref{fig:throughput_prop_fair_nonidealcs} the proportional fair throughput as in Figure \ref{fig:throughput_prop_fair} but with WiFi only deferring to LTE when no LTE/WiFi collision occurs at the start of the $T_{\rm on}$ period. Thus, assuming that WiFi only defers to LTE upon correct reception of the CTS-to-self.
Results in Figure \ref{fig:throughput_prop_fair_nonidealcs} show simulation and analytical results, the latter obtained using the analysis presented in the last subsection. It can be seen in Figure \ref{fig:throughput_prop_fair_nonidealcs}, that the throughput of WiFi remains practically unchanged. However, the LTE throughput is severely penalised for all configurations when using CSAT. The reason for this is the considerably higher collision probability of CSAT than LBE. Note also that LTE throughput is also reduced if compared to Figure \ref{fig:throughput_prop_fair} for LBE when $n=9$ due to the increase of collision probability with the number of WiFi stations. Although the throughput in this case is not as reduced as with CSAT, the performance degradation is considerable. One way to alleviate this in LBE is for the LTE to transmit before the DIFS to allow WiFi stations to decode the CTS-to-self, similarly as described in \textbf{add citation to victor's work-next week}.

\begin{figure*}[hhht!] 
\centering
\subfigure[$n=1,T_{\rm on}=10$ms]{\includegraphics[width=0.65\columnwidth]{./Figures/S_wifilte_n1_Ton10_ctstoself.eps}}
\subfigure[$n=3,T_{\rm on}=10$ms]{\includegraphics[width=0.65\columnwidth]{./Figures/S_wifilte_n3_Ton10_ctstoself.eps}}
\subfigure[$n=9,T_{\rm on}=10$ms]{\includegraphics[width=0.65\columnwidth]{./Figures/S_wifilte_n9_Ton10_ctstoself.eps}}\\
\subfigure[$n=1,T_{\rm on}=50$ms]{\includegraphics[width=0.65\columnwidth]{./Figures/S_wifilte_n1_Ton50_ctstoself.eps}}
\subfigure[$n=3,T_{\rm on}=50$ms]{\includegraphics[width=0.65\columnwidth]{./Figures/S_wifilte_n3_Ton50_ctstoself.eps}}
\subfigure[$n=9,T_{\rm on}=50$ms]{\includegraphics[width=0.65\columnwidth]{./Figures/S_wifilte_n9_Ton50_ctstoself.eps}}
\caption{Resulting throuhgput using the proportional fair allocation result with imperfect carrier sensing for different configurations of $n$ and $T_{\rm on}$ while varying $n_{\rm agg}$ (effectively changing the packet size of WiFi transmissions). Simulation results are averages of $100$ simulation runs with $50$ s time horizon.}
\label{fig:throughput_prop_fair_nonidealcs}
\end{figure*}


\vspace{0.3cm}
\fbox{\begin{minipage}{0.9\columnwidth}
\emph{To sum up, heterogeneity in the physical layers between coexisting technologies may prevent correct detection of scheduled transmissions by CSMA/CA nodes. To alleviate this, explicit signaling can be used. However, this signaling is prone to loss due to collisions, affecting the resulting throughput for the scheduled network.}
\end{minipage}}
\vspace{0.3cm}

%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Multiple LTE Networks}
%\textbf{**maybe NAV trick makes this easier ? does this create hidden terminal-like issues ?}


%\textbf{**do we assume LTE uses 20MHz bandwidth, or could it use less ?  if less then could pack LTE networks using frequency separation}

%\subsection{Collaborative Management}
%\textbf{**can LTE use its better view of channel conditions to manage carrier sense/hidden terminals better ?  Multiple LTE base-stations listening to channel, and clients also report to base-station. all are tightly time-synchronised if belong to same operator (part of LTE spec to help with handover and interference management).  }


